Geographic Spillover Effects of Prescription Drug Monitoring Programs (PDMPs)

Prescription Drug Monitoring Programs (PDMPs) seek to potentially reduce opioid misuse by restricting the sale of opioids in a state. We examine discontinuities along state borders, where one side may have a PDMP and the other side may not. We find that electronic PDMP implementation, whereby doctors and pharmacists can observe a patient's opioid purchase history, reduces a state's opioid sales but increases opioid sales in neighboring counties on the other side of the state border. We also find systematic differences in opioid sales and mortality between border counties and interior counties. These differences decrease when neighboring states both have ePDMPs, which is consistent with the hypothesis that individuals cross state lines to purchase opioids. Our work highlights the importance of understanding the opioid market as connected across counties or states, as we show that states are affected by the opioid policies of their neighbors.

==> table/Regression1.tex <==

\caption{Impact of PDMP laws on opioid sales}
\label{tab:reg1}
	
\begin{tabular} {L{0.25\textwidth}C{0.09\textwidth}C{0.09\textwidth}C{0.09\textwidth}C{0.09\textwidth}C{0.09\textwidth}}
\hline\hline
 &\multicolumn{5}{c}{Dependent variable:}\\\cline{2-6}
 &\multicolumn{5}{c}{Sales per person} \\
 & (1) & (2) & (3) & (4) & (5) \\\hline
 $\beta_1$ - PDMP law & -0.006***  &-0.007***&-0.004**&-0.004**&-0.004**\\
 & (0.001)  & (0.002) & (0.002) & (0.002)& (0.002)\\
 $\beta_2$ - Border county &  & & 0.006*** & 0.004***&0.002\\
 &&& (0.002) & (0.001)& (0.002)\\
 $\beta_3$ - Law x border & && -0.009*** & -0.008***&-0.010***\\
 &&& (0.002) & (0.002)& (0.003)\\
 $\beta_4$ - Nearby law x border&&&&&0.005***\\
 &&&&&(0.002)\\\hline
 County FE & Yes  &&&&&\\
 State FE & & Yes & Yes & Yes & Yes \\
 Year FE &  Yes & Yes & Yes & Yes & Yes \\
 Controls &&&& Yes & Yes\\\hline
 Observations &  26,154 & 26,154 & 26,154 & 26,154& 26,154\\
 $R^2$ & 0.001 & 0.458& 0.459 & 0.519 & 0.519\\\hline\hline
 
\end{tabular}

\begin{tablenotes}
	\small
	\item \textit{Notes:} TODO
\end{tablenotes}

==> table/Regression3.tex <==
\caption{Impact of PDMP laws and nearby laws on opioid sales and mortality}
\label{tab:reg3}
	
\begin{tabular} {L{0.2\textwidth}C{0.1\textwidth}C{0.1\textwidth}C{0.1\textwidth}C{0.1\textwidth}}
\hline\hline
 &\multicolumn{4}{c}{Dependent variable:}\\\cline{2-5}
 &\multicolumn{2}{c}{Sales} & \multicolumn{2}{c}{Mortality}\\
 & (1) & (2) & (3) & (4) \\\hline
 Inland x laws & -0.004* & -0.006*** & -0.349*** & -0.344*** \\
 & (0.002) &  (0.002) &  (0.076) &  (0.074)\\
 Border (0,0) &  0.007***  & 0.003*  & -0.418*** &-0.528*** \\
 &(0.002) &  (0.002)  & (0.071)  & (0.070)\\
 Border (0,1) & 0.003 &  -0.004** & -0.574***& -0.735***\\
 &(0.002) &  (0.002) &  (0.087) &  (0.085) \\
 Border (1,0) & -0.015***& -0.014*** &-1.095*** &-1.162*** \\
 &  (0.003) &  (0.002) &  (0.111) &  (0.108) \\
 Border (1,1) & -0.002 &   -0.002  & -0.516***& -0.458***\\
 &(0.002)  & (0.002) &  (0.098) &  (0.096) \\\hline
 State FE & Yes& Yes& Yes& Yes\\
 Year FE& Yes& Yes& Yes& Yes\\
 Controls&& Yes& & Yes\\\hline
 Observations & 26,154 & 26,154 & 26,154 & 26,154\\
 $R^2$ & 0.459   &  0.595  &   0.286   &  0.332\\\hline\hline
\end{tabular}

\begin{tablenotes}
	\small
	\item \textit{Notes:} LOL
\end{tablenotes}

==> table/reg1_enactdate.tex <==

\caption{Impact of PDMP laws on opioid sales using accepting information electronically date}
\label{tab:reg1_enactdate}
	
\begin{tabular} {L{0.25\textwidth}C{0.09\textwidth}C{0.09\textwidth}C{0.09\textwidth}C{0.09\textwidth}C{0.09\textwidth}C{0.09\textwidth}}
\hline\hline
 &\multicolumn{6}{c}{Dependent variable:}\\\cline{2-7}
 &\multicolumn{6}{c}{Sales per person} \\
 & (1) & (2) & (3) & (4) & (5) & (6) \\\hline
 PDMP law & 0.007*** & 0.007*** & 0.007*** & 0.005** & 0.005** & 0.005**\\
          & (0.001)  & (0.002) & (0.003) &(0.002)&(0.002)&(0.002)\\
 Border county & & & 0.002 & -0.003 & -0.0032 & 0.006*\\
 &&&                (0.002)& (0.002)& (0.003)& (0.003)\\
 Law x border & & & 0.0003 & 0.004* & 0.005* & -0.004 \\
 &&&               (0.003) &(0.002)&(0.002)& (0.004)\\
 Nearby law x border&&&&& -0.004** & -0.013***\\
 &&&&&                    (0.002)& (0.004)\\
 Nearby law x border x law&&&&&&0.012***\\
 &&&&&&(0.004)\\\hline
 County FE & Yes  &&&&&\\
 State FE & & Yes & Yes & Yes & Yes & Yes\\
 Year FE &  Yes & Yes & Yes & Yes & Yes & Yes \\
 Controls &&&& Yes & Yes & Yes\\\hline
 Observations &  26,154 & 26,154 & 26,154 & 26,154& 26,154& 26,154\\
 $R^2$ & 0.0001 & 0.458& 0.458 & 0.519 & 0.519 & 0.519\\\hline\hline
 
\end{tabular}

\begin{tablenotes}
	\small
	\item \textit{Notes:} TODO
\end{tablenotes}

==> table/reg1_rebustdate.tex <==

\caption{Impact of PDMP laws on opioid sales using PDMP enactment date (different source)}
\label{tab:reg1_robustdate}
	
\begin{tabular} {L{0.25\textwidth}C{0.09\textwidth}C{0.09\textwidth}C{0.09\textwidth}C{0.09\textwidth}C{0.09\textwidth}C{0.09\textwidth}}
\hline\hline
 &\multicolumn{6}{c}{Dependent variable:}\\\cline{2-7}
 &\multicolumn{6}{c}{Sales per person} \\
 & (1) & (2) & (3) & (4) & (5) & (6) \\\hline
 PDMP law & 0.006*** & 0.005** & 0.005** & 0.004 & 0.003 & 0.004\\
          & (0.001)  & (0.002) & (0.003) &(0.002)&(0.002)&(0.002)\\
 Border county & & & 0.002 & -0.003 & -0.002 & 0.016***\\
 &&&                (0.003)& (0.003)& (0.003)& (0.005)\\
 Law x border & & & 0.0001 & 0.004 & 0.004 & -0.019*** \\
 &&&               (0.003) &(0.003)&(0.003)& (0.005)\\
 Nearby law x border&&&&& -0.001 & -0.025***\\
 &&&&&                    (0.002)& (0.005)\\
 Nearby law x border x law&&&&&&0.029***\\
 &&&&&&(0.005)\\\hline
 County FE & Yes  &&&&&\\
 State FE & & Yes & Yes & Yes & Yes & Yes\\
 Year FE &  Yes & Yes & Yes & Yes & Yes & Yes \\
 Controls &&&& Yes & Yes & Yes\\\hline
 Observations &  26,154 & 26,154 & 26,154 & 26,154& 26,154& 26,154\\
 $R^2$ & 0.002 & 0.458& 0.458 & 0.519 & 0.519 & 0.519\\\hline\hline
 
\end{tabular}

\begin{tablenotes}
	\small
	\item \textit{Notes:} TODO
\end{tablenotes}

==> table/regression2.tex <==

\caption{Impact of PDMP laws on opioid mortality}
\label{tab:reg2}
	
\begin{tabular} {L{0.25\textwidth}C{0.09\textwidth}C{0.09\textwidth}C{0.09\textwidth}C{0.09\textwidth}C{0.09\textwidth}}
\hline\hline
 &\multicolumn{5}{c}{Dependent variable:}\\\cline{2-6}
 &\multicolumn{5}{c}{Mortality per 10,000 residents} \\
 & (1) & (2) & (3) & (4) & (5)\\\hline
 $\beta_1$ - PDMP law & -0.382*** & -0.345*** & -0.373*** & -0.400***&-0.370***\\
 &  (0.052) &  (0.071) &  (0.075)  & (0.073)  & (0.074) \\
 $\beta_2$ - Border county &  & & -0.462*** & -0.567*** & -0.666***\\
 &&&  (0.061)  & (0.061) & (0.068)\\
 $\beta_3$ - Law x border & && 0.096 & 0.189** & 0.118\\
 &&& (0.088) & (0.087) & (0.089)\\
 $\beta_4$ - Nearby law x border &&&&& 0.248***\\
 &&&&&(0.075)\\\hline
 County FE & Yes  &&&&\\
 State FE & & Yes & Yes & Yes & Yes\\
 Year FE &  Yes & Yes & Yes & Yes & Yes \\
 Controls &&&& Yes & Yes\\\hline
 Observations &  26,154 & 26,154 & 26,154 & 26,154& 26,154\\
 $R^2$ & &  0.283   &  0.286   &  0.318 &\\\hline\hline
 
\end{tabular}

\begin{tablenotes}
	\small
	\item \textit{Notes:} TODO
\end{tablenotes}

==> table_0615/endogeneity.tex <==

\caption{Endogeneity of PDMP adoption}
\label{tab:endogeneity}
	
\begin{tabular} {C{0.12\textwidth}C{0.12\textwidth}C{0.12\textwidth}C{0.12\textwidth}C{0.12\textwidth}}
\hline\hline
Law & Year & Has a law & \multicolumn{2}{c}{Does not have a law}\\
&&& will have in 3 & will not in 3\\\hline
PDMP&2006&0.094&0.155&0.116\\
PDMP&2010&0.192&0.203&0.155\\
ePDMP&2006&0.115&0.090&0.118\\
ePDMP&2010&0.154&0.238&0.204\\
MA-PDMP&2006&NA&0.145&0.106\\
MA-PDMP&2010&0.248&0.209&0.186\\

\hline\hline
 
\end{tabular}

\begin{tablenotes}
	\small
	\item \textit{Notes:} The table documents MME per person for states that does have a PDMP law by year $t$, states that do not but will have in the next 3 years, and states that do not and will not in the next 3 years. This table does not show our point cleanly, and Shiyu can't think of any other way to do this.
\end{tablenotes}
